Autoencoding Conditional GAN for Portfolio Allocation Diversification

Over the decades, the Markowitz framework has been used extensively in portfolio analysis though it puts too much emphasis on the analysis of the market uncertainty rather than on the trend prediction. While generative adversarial network (GAN) and conditional GAN (CGAN) have been explored to generate financial time series and extract features that can help portfolio analysis. The limitation of the CGAN framework stands in putting too much emphasis on generating series rather than keeping features that can help this generator. In this paper, we introduce an autoencoding CGAN (ACGAN) based on deep generative models that learns the internal trend of historical data while modeling market uncertainty and future trends. We evaluate the model on several real-world datasets from both the US and Europe markets, and show that the proposed ACGAN model leads to better portfolio allocation and generates series that are closer to true data compared to the existing Markowitz and CGAN approaches.

==> symbols.tex <==
% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\integer}{\mathbb{Z}}
%\newcommand{\det}{\mathrm{det}}

\newcommand{\cspace}{\mathcal{C}}
\newcommand{\nspace}{\mathcal{N}}

\newcommand{\leadto}{\qquad\underrightarrow{ \text{leads to} }\qquad}
\newcommand{\leadtosmall}{\,\,\underrightarrow{ \text{leads to} }\,\,}


%%%% NEW DEFINITIONS %%%%%

\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Exp}{\mathrm{E}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\gap}{\,\,\,\,\,\,\,\,}


\newcommand{\exampbar}{\hfill $\square$\par}

%\newcommand{\bC}{\mat{C}}
%\newcommand{\ba}{\vec{a}}
%\newcommand{\bC}{\mathbf{C}}

%% begin new command fo clustering
\newcommand{\bOmega}{\boldsymbol\Omega}
\newcommand{\bomega}{\boldsymbol\omega}
\newcommand{\balpha}{\boldsymbol\alpha}
\newcommand{\bbeta}{\boldsymbol\beta}
\newcommand{\bdelta}{\boldsymbol\delta}
\newcommand{\btheta}{\boldsymbol\theta}
\newcommand{\bTheta}{\boldsymbol\Theta}
\newcommand{\bPhi}{\boldsymbol\Phi}
\newcommand{\bPsi}{\boldsymbol\Psi}
\newcommand{\bpsi}{\boldsymbol\psi}
\newcommand{\bgamma}{\boldsymbol\gamma}
\newcommand{\bepsilon}{\boldsymbol\epsilon}
\newcommand{\bLambda}{\boldsymbol\Lambda}
\newcommand{\boldeta}{\boldsymbol\eta}
\newcommand{\blambda}{\boldsymbol\lambda}
\newcommand{\bphi}{\boldsymbol\phi}
\newcommand{\bphiast}{\bphi_\ast}
\newcommand{\bmu}{\boldsymbol\mu}
\newcommand{\bsigma}{\boldsymbol\sigma}
\newcommand{\bSigma}{\boldsymbol\Sigma}


\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\diag}{\mathrm{diag}}


\newcommand{\dotL}{\dot{\bm{L}}}
\newcommand{\dotU}{\dot{\bm{U}}}
\newcommand{\ddotL}{\ddot{\bm{L}}}


%\newcommand{\widetildebG}{\widetilde{\bm{G}}}
%\newcommand{\widetildebV}{\widetilde{\bm{V}}}
%\newcommand{\widetildebU}{\widetilde{\bm{U}}}
%\newcommand{\widetildebv}{\widetilde{\bm{v}}}
\newcommand{\widebarbA}{\overline{\bm{A}}}
\newcommand{\widebarbB}{\overline{\bm{B}}}
\newcommand{\widebarbC}{\overline{\bm{C}}}
\newcommand{\widebarbD}{\overline{\bm{D}}}
\newcommand{\widebarbE}{\overline{\bm{E}}}
\newcommand{\widebarbF}{\overline{\bm{F}}}
\newcommand{\widebarbG}{\overline{\bm{G}}}
\newcommand{\widebarbH}{\overline{\bm{H}}}
\newcommand{\widebarbI}{\overline{\bm{I}}}
\newcommand{\widebarbJ}{\overline{\bm{J}}}
\newcommand{\widebarbK}{\overline{\bm{K}}}
\newcommand{\widebarbL}{\overline{\bm{L}}}
\newcommand{\widebarbM}{\overline{\bm{M}}}
\newcommand{\widebarbN}{\overline{\bm{N}}}
\newcommand{\widebarbO}{\overline{\bm{O}}}
\newcommand{\widebarbP}{\overline{\bm{P}}}
\newcommand{\widebarbQ}{\overline{\bm{Q}}}
\newcommand{\widebarbR}{\overline{\bm{R}}}
\newcommand{\widebarbS}{\overline{\bm{S}}}
\newcommand{\widebarbT}{\overline{\bm{T}}}
\newcommand{\widebarbU}{\overline{\bm{U}}}
\newcommand{\widebarbV}{\overline{\bm{V}}}
\newcommand{\widebarbW}{\overline{\bm{W}}}
\newcommand{\widebarbX}{\overline{\bm{X}}}
\newcommand{\widebarbY}{\overline{\bm{Y}}}
\newcommand{\widebarbZ}{\overline{\bm{Z}}}
\newcommand{\widebarba}{\overline{\bm{a}}}
\newcommand{\widebarbb}{\overline{\bm{b}}}
\newcommand{\widebarbc}{\overline{\bm{c}}}
\newcommand{\widebarbd}{\overline{\bm{d}}}
\newcommand{\widebarbe}{\overline{\bm{e}}}
\newcommand{\widebarbf}{\overline{\bm{f}}}
\newcommand{\widebarbg}{\overline{\bm{g}}}
\newcommand{\widebarbh}{\overline{\bm{h}}}
\newcommand{\widebarbi}{\overline{\bm{i}}}
\newcommand{\widebarbj}{\overline{\bm{j}}}
\newcommand{\widebarbk}{\overline{\bm{k}}}
\newcommand{\widebarbl}{\overline{\bm{l}}}
\newcommand{\widebarbm}{\overline{\bm{m}}}
\newcommand{\widebarbn}{\overline{\bm{n}}}
\newcommand{\widebarbo}{\overline{\bm{o}}}
\newcommand{\widebarbp}{\overline{\bm{p}}}
\newcommand{\widebarbq}{\overline{\bm{q}}}
\newcommand{\widebarbr}{\overline{\bm{r}}}
\newcommand{\widebarbs}{\overline{\bm{s}}}
\newcommand{\widebarbt}{\overline{\bm{t}}}
\newcommand{\widebarbu}{\overline{\bm{u}}}
\newcommand{\widebarbv}{\overline{\bm{v}}}
\newcommand{\widebarbw}{\overline{\bm{w}}}
\newcommand{\widebarbx}{\overline{\bm{x}}}
\newcommand{\widebarby}{\overline{\bm{y}}}
\newcommand{\widebarbz}{\overline{\bm{z}}}


\newcommand{\widetildebA}{\widetilde{\bm{A}}}
\newcommand{\widetildebB}{\widetilde{\bm{B}}}
\newcommand{\widetildebC}{\widetilde{\bm{C}}}
\newcommand{\widetildebD}{\widetilde{\bm{D}}}
\newcommand{\widetildebE}{\widetilde{\bm{E}}}
\newcommand{\widetildebF}{\widetilde{\bm{F}}}
\newcommand{\widetildebG}{\widetilde{\bm{G}}}
\newcommand{\widetildebH}{\widetilde{\bm{H}}}
\newcommand{\widetildebI}{\widetilde{\bm{I}}}
\newcommand{\widetildebJ}{\widetilde{\bm{J}}}
\newcommand{\widetildebK}{\widetilde{\bm{K}}}
\newcommand{\widetildebL}{\widetilde{\bm{L}}}
\newcommand{\widetildebM}{\widetilde{\bm{M}}}
\newcommand{\widetildebN}{\widetilde{\bm{N}}}
\newcommand{\widetildebO}{\widetilde{\bm{O}}}
\newcommand{\widetildebP}{\widetilde{\bm{P}}}
\newcommand{\widetildebQ}{\widetilde{\bm{Q}}}
\newcommand{\widetildebR}{\widetilde{\bm{R}}}
\newcommand{\widetildebS}{\widetilde{\bm{S}}}
\newcommand{\widetildebT}{\widetilde{\bm{T}}}
\newcommand{\widetildebU}{\widetilde{\bm{U}}}
\newcommand{\widetildebV}{\widetilde{\bm{V}}}
\newcommand{\widetildebW}{\widetilde{\bm{W}}}
\newcommand{\widetildebX}{\widetilde{\bm{X}}}
\newcommand{\widetildebY}{\widetilde{\bm{Y}}}
\newcommand{\widetildebZ}{\widetilde{\bm{Z}}}
\newcommand{\widetildeba}{\widetilde{\bm{a}}}
\newcommand{\widetildebb}{\widetilde{\bm{b}}}
\newcommand{\widetildebc}{\widetilde{\bm{c}}}
\newcommand{\widetildebd}{\widetilde{\bm{d}}}
\newcommand{\widetildebe}{\widetilde{\bm{e}}}
\newcommand{\widetildebf}{\widetilde{\bm{f}}}
\newcommand{\widetildebg}{\widetilde{\bm{g}}}
\newcommand{\widetildebh}{\widetilde{\bm{h}}}
\newcommand{\widetildebi}{\widetilde{\bm{i}}}
\newcommand{\widetildebj}{\widetilde{\bm{j}}}
\newcommand{\widetildebk}{\widetilde{\bm{k}}}
\newcommand{\widetildebl}{\widetilde{\bm{l}}}
\newcommand{\widetildebm}{\widetilde{\bm{m}}}
\newcommand{\widetildebn}{\widetilde{\bm{n}}}
\newcommand{\widetildebo}{\widetilde{\bm{o}}}
\newcommand{\widetildebp}{\widetilde{\bm{p}}}
\newcommand{\widetildebq}{\widetilde{\bm{q}}}
\newcommand{\widetildebr}{\widetilde{\bm{r}}}
\newcommand{\widetildebs}{\widetilde{\bm{s}}}
\newcommand{\widetildebt}{\widetilde{\bm{t}}}
\newcommand{\widetildebu}{\widetilde{\bm{u}}}
\newcommand{\widetildebv}{\widetilde{\bm{v}}}
\newcommand{\widetildebw}{\widetilde{\bm{w}}}
\newcommand{\widetildebx}{\widetilde{\bm{x}}}
\newcommand{\widetildeby}{\widetilde{\bm{y}}}
\newcommand{\widetildebz}{\widetilde{\bm{z}}}




\newcommand{\off}{\text{off}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bd}{\bm{d}}
\newcommand{\bD}{\bm{D}}
\newcommand{\be}{\bm{e}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bff}{\bm{f}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bi}{\bm{i}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bq}{\bm{q}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bX}{\bm{X}}
\newcommand{\by}{\bm{y}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bZ}{\bm{Z}}



\newcommand{\abovebX}[1]{\overset{\mathit{(#1)}}{\bX}}


\newcommand{\eG}{\bm{\mathscr{G}}}
\newcommand{\eA}{\bm{\mathscr{A}}}
\newcommand{\eB}{\bm{\mathscr{B}}}
\newcommand{\eY}{\bm{\mathscr{Y}}}
\newcommand{\eX}{\bm{\mathscr{X}}}
\newcommand{\eL}{\bm{\mathscr{L}}}
\newcommand{\weX}{\widehat{\bm{\mathscr{X}}}}
\newcommand{\weG}{\widehat{\bm{\mathscr{G}}}}

\newcommand{\widehatbA}{\widehat{\bm{A}}}

\newcommand{\mathcalV}{\mathcal{V}}
\newcommand{\dist}{\mathrm{dist}}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\kernel}{\mathbf{ker}}
\newcommand{\mathE}{\mathbb{E}}


\newcommand{\mat}[1]{\mathbf{#1}}
\renewcommand\vec{\mathbf}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\trans}[1]{\ensuremath{#1^{ \top}}}

% biconjugate decomposition
\newcommand{\brx}{\bm{R}_\gamma^{(x)}}
\newcommand{\bry}{\bm{R}_\gamma^{(y)}} 
\newcommand{\brxt}{\bm{R}_\gamma^{(x)\top}}
\newcommand{\bryt}{\bm{R}_\gamma^{(y)\top}} 
\newcommand{\bxgamma}{\bX_\gamma}
\newcommand{\bygamma}{\bY_\gamma}
\newcommand{\bugamma}{\bU_\gamma}
\newcommand{\bvgamma}{\bV_\gamma}
\newcommand{\bomegagamma}{\bOmega_\gamma}
\newcommand{\svd}{\mathrm{svd}}
